Radiation power and linewidth of a semifluxon-based Josephson oscillator

We demonstrate a high-frequency generator operating at ~200GHz based on flipping a semifluxon in a Josephson junction of moderate normalized length. The semifluxon spontaneously appears at the $\pi$ discontinuity of the Josephson phase artificially created by means of two tiny current injectors. The radiation is detected by an on-chip detector (tunnel junction). The estimated radiation power (at the detector) is ~8nW and should be compared with the dc power of ~100nW consumed by the generator. The measured radiation linewidth, as low as 1.1MHz, is typical for geometrical (Fiske) resonances although we tried to suppress such resonances by placing well-matched microwave transformers at its both ends. Making use of a phase-locking feedback loop we are able to reduce the radiation linewidth to less than 1Hz measured relative to the reference oscillator and defined just by the resolution of our measurement setup.

==> MyMc.tex <==
%%% This is 'MyMc.tex' v3.00
%%% LaTeX macros for frequently used abbreviations
%%% 13.12.2011 by Edward Goldobin <gold@uni-tuebingen.de>

\RequirePackage{xspace}

%stupid macros like \ie, \eg, \etc
\newcommand{\ie}{\textit{i.e.}\xspace}
\newcommand{\eg}{\textit{e.g.}\xspace}
\newcommand{\etal}{\textit{et al.}\xspace}
\newcommand{\cf}{\textit{cf.}\xspace}
\newcommand{\vs}{\textit{vs.}\xspace}
\newcommand{\etc}{\textit{etc.}\xspace}
\newcommand{\viz}{\textit{viz.}\xspace}
%\newcommand{\etal}{\textit{et~al.}\xspace}
\newcommand{\lhs}{l.h.s.\xspace}
\newcommand{\rhs}{r.h.s.\xspace}

\newcommand{\mum}{\ensuremath{\mathrm{\mu m}}}
\newcommand{\degree}{\ensuremath{^\circ}\xspace}

%units
\newcommand{\units}[1]{\ensuremath{\,\mathrm{#1}}}


% Convenient ratios and (partial) derivatives
%
%big \frac is called \ratio.
%usage: \ratio{a}{b}
\newcommand{\ratio}[2]{\displaystyle\frac{#1}{#2}}
%usage: \fracd{y}{x} produces fraction dy/dx.
%usage with optional argument: \fracd[2]{y}{x} produces 2nd derivative
\newcommand{\fracd}[3][]{\displaystyle\frac{d^{#1}#2}{d#3^{#1}}}
%usage: \fracp{y}{x} produces partial derivatice dy/dx.
%usage with optional argument: \fracp[2]{y}{x} produces 2nd order partial derivative
\newcommand{\fracp}[3][]{\displaystyle\frac{\partial^{#1}#2}{\partial#3^{#1}}}
%mixed derivatives are not implemented yet :-(

%Averaging macros:
%
%usage1: \av{V} - averaged V
%usage2: \av[x]{V} - V averaged with respect to x
\newcommand{\av}[2][]{\ensuremath{\left\langle#2\right\rangle}_{#1}\xspace}
%usage: \mean{u} - produced bar over the argument
\newcommand{\mean}[1]{\ensuremath{\overline{#1}}\xspace}
\newcommand{\dev}[2][]{\ensuremath{\widetilde{#2}_{#1}}\xspace}

%Freq used materials
\RequirePackage{xspace}
\newcommand{\YBCO}{YBa$_2$Cu$_3$O$_7$\xspace}
\newcommand{\LBCO}[1][x]{La$_{2-#1}$Ba$_#1$CuO$_4$\xspace}
\newcommand{\BSCCO}{Bi$_2$Sr$_2$Ca$_1$Cu$_2$O$_{8}$\xspace}
\newcommand{\NBCO}[1][x]{NdBa$_2$Cu$_3$O$_{7-#1}$\xspace}
\newcommand{\TBCO}{Tl$_2$Ba$_2$CuO$_6$\xspace}
\newcommand{\HBCO}{HgBa$_2$CuO$_6$\xspace}
\newcommand{\NCCO}{Nd$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\PCCO}{Pr$_{2-x}$Ce$_x$CuO$_4$\xspace}
\newcommand{\LCMO}[1][x]{La$_{1-#1}$Ca$_x$MnO$_3$\xspace}
\newcommand{\STO}{SrTiO$_3$\xspace}
\newcommand{\CeO}{CeO$_2$\xspace}
\newcommand{\MgB}{MgB$_2$\xspace}
\newcommand{\OrgIJJ}{$\kappa$-(BEDT-TTF)$_2$Cu(NCS)$_2$\xspace}


%technology definitions
\newcommand{\NbAlOxNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechNb}{Nb-AlO$_x$-Nb\xspace}
\newcommand{\TechYBCONb}{YBCO-Nb\xspace}
%
\newcommand{\SIS}{\ensuremath{\mathrm{S|I|S}}\xspace}
\newcommand{\SNS}{\ensuremath{\mathrm{S|N|S}}\xspace}
\newcommand{\SFS}{\ensuremath{\mathrm{S|F|S}}\xspace}
\newcommand{\SIFS}{S$|$I$|$F$|$S\xspace}
\newcommand{\SfiS}{S$|$FI$|$S\xspace}
%\newcommand{\SJS}{\ensuremath{\mathrm{S-FI-S}}\xspace}

%%
%% Freq used math symbols
%%

%Elliptic fns
\newcommand{\am}{\mathop{\mathrm{am}}\nolimits}
\newcommand{\dn}{\mathop{\mathrm{dn}}\nolimits}
\newcommand{\sn}{\mathop{\mathrm{sn}}\nolimits}
\newcommand{\cn}{\mathop{\mathrm{cn}}\nolimits}
\newcommand{\gd}{\mathop{\mathrm{gd}}\nolimits}
\newcommand{\E} {\mathop{\mathrm{E}}\nolimits}
\newcommand{\F} {\mathop{\mathrm{F}}\nolimits}
\newcommand{\K} {\mathop{\mathrm{K}}\nolimits}
\newcommand{\J}[1][] {\mathop{\mathrm{J_{#1}}}\nolimits}
\newcommand{\Ai} {\mathop{\mathrm{Ai}}\nolimits}
\newcommand{\Bi} {\mathop{\mathrm{Bi}}\nolimits}

%Other fns
%\newcommand{\const}{\mathop{const}\nolimits}
\newcommand{\atanh}{\mathop{\mathrm{atanh}}\nolimits}
\newcommand{\acot}{\mathop{\mathrm{acot}}\nolimits}
\newcommand{\sech}{\mathop{\mathrm{sech}}\nolimits}
\newcommand{\sgn}{\mathop{\mathrm{sgn}}\nolimits}
\newcommand{\floor}{\mathop{\mathrm{floor}}\nolimits}
\newcommand{\const}{\mathop{\mathrm{const}}\nolimits}
\renewcommand{\Re}{\mathop{\mathrm{Re}}\nolimits}
\renewcommand{\Im}{\mathop{\mathrm{Im}}\nolimits}
%\newcommand{\Det}{\mathop{\mathrm{det}}\nolimits}
%\newcommand{\Tr}{\mathop{\mathrm{Tr}}\nolimits}

\newcommand{\qstate}[1]{\ensuremath{\left\lvert\state{#1}\right\rangle}}
\newcommand{\rot}{\mathop\mathrm{\mathbf{rot}}\nolimits}
\newcommand{\grad}{\mathop\mathbf{{\rm grad}}\nolimits}
%\newcommand{\div}{\mathop{{\rm div}}\nolimits}


%just shortcuts
%\newcommand{\HS}{\ensuremath{{\cal H}}}
\newcommand{\Heavyside}{\mathop{\mathrm{H}}\nolimits}
\newcommand{\G}{\ensuremath{{\cal G}}}
\newcommand{\Dx}{\ensuremath{{\Delta x}}}
\newcommand{\dx}{\ensuremath{{\delta x}}}
\newcommand{\Dw}{\ensuremath{{\Delta w}}}
\newcommand{\D}[1]{\ensuremath{{\Delta #1}}}
%\newcommand{\d}[1]{\ensuremath{{\delta #1}}}

%\iffalse%{
\RequirePackage{amssymb}

% macros for showing/hiding corrections

%\RequirePackage[normalem]{ulem}

%\newcommand{\new}[1]{\textcolor{blue}{#1}}
%\newcommand{\del}[1]{\textcolor{red}{\sout{#1}}}
%\newcommand{\chg}[1]{\textcolor{magenta}{#1}}
\RequirePackage{ifthen}
\newboolean{ShowCorrections}
\setboolean{ShowCorrections}{true}%<-- set here show/notshow corrections

%%%Reduction/Corrections macros
\ifthenelse{\boolean{ShowCorrections}}{%
\usepackage[normalem]{ulem}%
\newcommand{\new}[1]{\textcolor[rgb]{0,0,1}{#1}}%
\newcommand{\old}[1]{\textcolor[rgb]{1,0,0}{\sout{#1}}}%
}{%
\newcommand{\new}[1]{#1}%
\newcommand{\old}[1]{}%
}


%%
%% Not allowed stuff
%%

%state command which may not translate correctly
\newcommand{\stat}[1]{\state{#1}}

%%tth:\def\relax{}
%%tth:\def\message#1{}

%\tracingmacros=2
%%%%%%%%%%

\def\state#1{\ensuremath{\stt#1.}}
\def\stt#1{%
\if#1.
\let\next=\relax
\else
  \if#1u
    \upharpoonleft%\uparrow
  \else\if#1d
    \downharpoonleft%\downarrow
  \else\if#1U
    \upharpoonright%\Uparrow
  \else\if#1D
    \downharpoonright%\Downarrow
  \else\if#1F
    \Uparrow
  \else\if#1A
    \Downarrow
  \else\if#1s
    \uparrow
  \else\if#1a
    \downarrow
  \else\if#1r
    \rightarrow
  \else\if#1l
    \leftarrow
  \else\if#1R
    \Rightarrow
  \else\if#1L
    \Leftarrow
  \else\if#1>
    \longrightarrow
  \else\if#1<
    \longleftarrow
  \else\if#1
  \relax
  \else
  ?\message{Unknown symbol #1 in the argument of macro state}
  \fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi\fi
\let\next=\stt
\fi
\next
}

%usage: \hstruct{Nb|Al|Nb}
%at the moment cannot accept math or lower indices. :-(
\def\hstruct#1{%
\let\accu=\relax%
\hstruc#1.%
\accu
}
\def\hstruc#1{%
\if#1.%end?
\let\next=\relax
\else
  \if#1|%
    \let\accu=\accu$|$%
%  \else\if#1
%    \relax
  \else
    \let\accu=\accu #1%\message{Unknown symbol #1 in the argument of macro \hstruc}
  \fi%\fi
  \let\next=\hstruc
\fi
\next
}


\newcounter{CurrTimeHH}\newcounter{CurrTimeMM}
\newcommand{\CurrTime}{%
  \setcounter{CurrTimeHH}{\time/60}%
  \setcounter{CurrTimeMM}{\time - \value{CurrTimeHH}*60}%
  \ifthenelse{\value{CurrTimeHH}<10}{0}{}\theCurrTimeHH:%
  \ifthenelse{\value{CurrTimeMM}<10}{0}{}\theCurrTimeMM%
}




==> we.tex <==
%Misc. macros to discuss with co-authors
\RequirePackage{color}
\newcommand{\EG}[1]{{\textcolor[rgb]{1,.4,0}{\textbf{EG:``#1''}}}}
\newcommand{\DK}[1]{{\textcolor[rgb]{0,0.7,0}{\textbf{DK:``#1''}}}}
\newcommand{\RK}[1]{{\textcolor[rgb]{1.0,0,0}{\textbf{RK:``#1''}}}}

\newcommand{\VK}[1]{{\textcolor[rgb]{0.4,.4,1}{\textbf{VK:``#1''}}}}
\newcommand{\MP}[1]{{\textcolor{red}{\textbf{MP:``#1''}}}}

